Adapting Foundation Models for Few-Shot Medical Image Segmentation: Actively and Sequentially

Recent advances in foundation models have brought promising results in computer vision, including medical image segmentation. Fine-tuning foundation models on specific low-resource medical tasks has become a standard practice. However, ensuring reliable and robust model adaptation when the target task has a large domain gap and few annotated samples remains a challenge. Previous few-shot domain adaptation (FSDA) methods seek to bridge the distribution gap between source and target domains by utilizing auxiliary data. The selection and scheduling of auxiliaries are often based on heuristics, which can easily cause negative transfer. In this work, we propose an Active and Sequential domain AdaPtation (ASAP) framework for dynamic auxiliary dataset selection in FSDA. We formulate FSDA as a multi-armed bandit problem and derive an efficient reward function to prioritize training on auxiliary datasets that align closely with the target task, through a single-round fine-tuning. Empirical validation on diverse medical segmentation datasets demonstrates that our method achieves favorable segmentation performance, significantly outperforming the state-of-the-art FSDA methods, achieving an average gain of 27.75% on MRI and 7.52% on CT datasets in Dice score. Code is available at the git repository: https://github.com/techicoco/ASAP.

==> figures/intro.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.85\linewidth,scale=1]{figures/in.pdf}
    \vspace{-0.2cm}
    \caption{Leveraging a wealth of public medical resources, including foundation models and available auxiliary datasets, our objective is to efficiently utilize these resources to tailor a model for the desired few-shot target task, shown in green.}
    \label{intro}
\vspace{-0.5cm}
\end{figure}

==> table/ASAP_CT.tex <==
\vspace{-0.1cm}
\begin{table}[!]
	\centering
%\begin{minipage}{0.95\linewidth}
\centering
\setlength\tabcolsep{4pt} 
\footnotesize
\caption{Results of different domain adaptation strategies on CT datasets. The segmentation evaluation metrics are the Dice score and the mean IoU score. Bold number: best score.}
\vspace{-0.2cm}
\label{ASAP_CT}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc|cc|cc}
\toprule
\multirow{2}{*}{Target} & \multirow{2}{*}{Method}
 & \multicolumn{2}{c}{UNet} & \multicolumn{2}{c}{SwinUNet} & \multicolumn{2}{c}{MambaUNet} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
 & & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
 & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
 & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}\\
\cmidrule(lr){1-8}
\multirow{5}{*}{Vessel} & Direct FT & 48.70 & 33.13 & 41.31 & 26.64 & 49.08 & 33.39\\ 
 & GMS (NIPS' 20) & 48.74 & 33.85 & 36.16 & 22.51 & 46.62 & 40.94 \\
 & MTL (MIA' 23) & 22.64 & 13.12 & 32.23 & 19.58 & 35.05 & 21.86 \\
& DAL (NIPS' 24) & 45.78 & 30.33 & 41.24 & 26.81 & 44.54 & 30.91 \\ 
\cmidrule{2-8}
 & ASAP (Ours) & \textbf{49.22} & \textbf{33.55} & \textbf{48.05} & \textbf{32.81}
 & \textbf{49.27} & \textbf{33.34}\\
\cmidrule(lr){1-8}
\cmidrule(lr){1-8}
\multirow{5}{*}{Liver} & Direct FT & 79.79 & 66.97 & 84.86 & 74.63 & 84.40 & 73.67\\ 
 & GMS (NIPS' 20) & 90.88 & 83.50 & 86.99 & 77.53 & 90.04 & 82.20 \\
 & MTL (MIA' 23) & 81.15 & 71.52 & 85.56 & 75.80 & 91.26 & 84.11 \\
& DAL (NIPS' 24) & 91.66 & 84.22 & 84.06 & 73.05 & 87.71 & 78.50 \\ 
\cmidrule{2-8}
 & ASAP (Ours) & \textbf{92.10} & \textbf{85.61} & \textbf{87.27} & \textbf{78.67}
 & \textbf{92.91} & \textbf{86.95}\\
 \bottomrule
\end{tabular}
}
%\end{minipage}
\vspace{-0.3cm}
\end{table}

==> table/ASAP_MRI.tex <==
\vspace{-0.1cm}
\begin{table}[!]
	\centering
%\begin{minipage}{0.95\linewidth}
\centering
\setlength\tabcolsep{4pt} 
\footnotesize
\caption{Results of different domain adaptation strategies on MRI datasets. The segmentation evaluation metrics are the Dice score and the mean IoU score. Bold number: best score.}
\vspace{-0.2cm}
\label{ASAP_MRI}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc|cc|cc}
\toprule
\multirow{2}{*}{Target} & \multirow{2}{*}{Method}
 & \multicolumn{2}{c}{UNet} & \multicolumn{2}{c}{SwinUNet} & \multicolumn{2}{c}{MambaUNet} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
 & & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
 & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
 & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}\\
\cmidrule(lr){1-8}
\multirow{5}{*}{PVL} & Direct FT & 23.48 & 13.82 & 18.35 & 10.48 & 27.20 & 16.18\\ 
 & GMS (NIPS' 20) & 23.50 & 13.56 & 20.41 & 11.86 & 27.45 & 16.72 \\
 & MTL (MIA' 23) & 20.79 & 11.70 & 14.62 & 8.41 & 19.02 & 11.09 \\
& DAL (NIPS' 24) & 26.76 & 15.99 & 19.65 & 11.26 & 26.92 & 16.23 \\ 
\cmidrule{2-8}
 & ASAP (Ours) & \textbf{27.95} & \textbf{16.80} & \textbf{22.16} & \textbf{13.02}
 & \textbf{30.06} & \textbf{18.48}\\
\cmidrule(lr){1-8}
\cmidrule(lr){1-8}
\multirow{5}{*}{WMH} & Direct FT & 57.03 & 40.78 & 64.24 & 48.79 & 62.35 & 45.51\\ 
 & GMS (NIPS' 20) & 52.86 & 39.40 & 64.54 & 50.91 & 65.78 & 50.36 \\
 & MTL (MIA' 23) & 58.13 & 41.29 & 53.69 & 38.83 & 53.81 & 38.76 \\
& DAL (NIPS' 24) & 62.74 & 46.75 & 67.16 & 51.47 & 63.62 & 48.68 \\ 
\cmidrule{2-8}
 & ASAP (Ours) & \textbf{66.94} & \textbf{53.10} & \textbf{67.62} & \textbf{52.04}
 & \textbf{71.06} & \textbf{56.04}\\
 \bottomrule
\end{tabular}
}
%\end{minipage}
\vspace{-0.3cm}
\end{table}

==> table/efficiency.tex <==
\begin{table}[!]
	\centering
%\begin{minipage}{0.95\linewidth}
\centering
\setlength\tabcolsep{4pt} 
\footnotesize
\caption{Efficiency study of different adaptation training strategies. The evaluation metrics are segmentation performance, i.e., the Dice score, and costs, i.e., training time. The results are the averages of all datasets. Bold number: best score.}
\vspace{-0.1cm}
\label{efficiency}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{UNet} & \multicolumn{2}{c}{SwinUNet} & \multicolumn{2}{c}{MambaUNet}\\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
 & {Dice (\%)} & Cost (h) 
 & {Dice (\%)} & Cost (h)
 & {Dice (\%)} & Cost (h)
 \\
% instead of \midrule. use \cline in booktabs
\cmidrule{1-7}
Direct FT & 53.01 & \textbf{1.76} & 53.01 & \textbf{1.76}\\ 
NAL (NIPS' 20) & 54.47 & 6.13 & 54.47 & 6.13\\
MTL (MIA' 23) & 52.77 & 63.57 & 52.77 & 63.5\\
DAL (NIPS' 24) & 58.14 & 7.40 & 58.14 & 7.40\\
\cmidrule{1-7}
ASAP (Ours) & \textbf{63.29} & 7.08 & \textbf{63.29} & 7.08
& \textbf{63.29} & 7.08\\
\bottomrule
\end{tabular}
}
%\end{minipage}
\vspace{-0.2cm}
\end{table}

==> table/unet.tex <==
\begin{table}[!]
\vspace{-0.3cm}
	\centering
%\begin{minipage}{0.95\linewidth}
\centering
\setlength\tabcolsep{4pt} 
\footnotesize
\caption{Results of different domain adaptation strategies on CT datasets. The segmentation evaluation metrics are the Dice score and the mean IoU score. Bold number: best score.}
\vspace{-0.2cm}
\label{ASAP_CT}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc|cc|cc}
\toprule
\multirow{2}{*}{Method}
 & \multicolumn{2}{c}{UNet} & \multicolumn{2}{c}{SwinUNet} & \multicolumn{2}{c}{MambaUNet} \\
 \cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
& \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
 & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
 & \multicolumn{1}{c}{Dice (\%)} & \multicolumn{1}{c}{mIoU (\%)}
\\
\cmidrule(lr){1-7}
Direct FT & 27.57 & 16.63 & 57.03 & 40.78  & 27.57 & 16.63 \\ 
NAL (NIPS' 20) & 33.66 & 22.22 & 52.86 & 39.40 & 60.94 & 46.08  \\
MTL (MIA' 23) & 23.48 & 13.82  & 58.13 & 41.29  & 61.08 & 48.99 \\
DAL (NIPS' 24) & 31.71 & 23.80  & 62.74 & 46.75  &  62.39 & 48.16\\ 
\cmidrule{1-7}
ASAP (Ours) & \textbf{40.61} & \textbf{27.05}  & \textbf{66.94} & \textbf{53.10}  &  \textbf{67.80} & \textbf{52.63} \\
% Direct FT & 57.03 & 40.78  & 27.57 & 16.63  & 59.11 & 44.31  & 68.33 & 53.66 \\ 
% NAL (NIPS' 20) & 52.86 & 39.40  & 33.66 & 22.22   & 60.94 & 46.08   & 70.43 & 55.60 \\
% MTL (MIA' 23) & 58.13 & 41.29  & 23.48 & 13.82  & 61.08 & 48.99  & 68.38 & 53.37 \\
% DAL (NIPS' 24) & 62.74 & 46.75  & 31.71 & 23.80  & 62.39 & 48.16 & 75.72 & 61.22 \\ 
% DTW (ICLR' 21) & 59.11 & 44.31  & 29.30  & 18.99 & 62.74 & 46.75 & 73.92 & 58.11\\
% \cmidrule{1-9}
% ASAP (Ours) & \textbf{66.94} & \textbf{53.10}  & \textbf{42.61} & \textbf{28.05}  & \textbf{67.80} & \textbf{52.63}  & \textbf{75.81} & \textbf{61.25}\\
\bottomrule
\end{tabular}
}
%\end{minipage}
\vspace{-0.2cm}
\end{table}
